What Can Database Query Processing Do for Instance-Spanning Constraints?

In the last decade, the term instance-spanning constraint has been introduced in the process mining field to refer to constraints that span multiple process instances of one or several processes. Of particular relevance, in this setting, is checking whether process executions comply with constraints of interest, which at runtime calls for suitable monitoring techniques. Even though event data are often stored in some sort of database, there is a lack of database-oriented approaches to tackle compliance checking and monitoring of (instance-spanning) constraints. In this paper, we fill this gap by showing how well-established technology from database query processing can be effectively used for this purpose. We propose to define an instance-spanning constraint through an ensemble of four database queries that retrieve the satisfying, violating, pending-satisfying, and pending-violating cases of the constraint. In this context, the problem of compliance monitoring then becomes an application of techniques for incremental view maintenance, which is well-developed in database query processing. In this paper, we argue for our approach in detail, and, as a proof of concept, present an experimental validation using the DBToaster incremental database query engine.

==> pl.tex <==
% --- ugly internals for language definition ---
%
\makeatletter

% initialisation of user macros
\newcommand\PrologPredicateStyle{}
\newcommand\PrologVarStyle{}
\newcommand\PrologAnonymVarStyle{}
\newcommand\PrologAtomStyle{}
\newcommand\PrologOtherStyle{}
\newcommand\PrologCommentStyle{}

% useful switches (to keep track of context)
\newif\ifpredicate@prolog@
\newif\ifwithinparens@prolog@

% save definition of underscore for test
\lst@SaveOutputDef{`_}\underscore@prolog

% local variables
\newcount\currentchar@prolog

\newcommand\@testChar@prolog%
{%
  % if we're in processing mode...
  \ifnum\lst@mode=\lst@Pmode%
    \detectTypeAndHighlight@prolog%
  \else
    % ... or within parentheses
    \ifwithinparens@prolog@%
      \detectTypeAndHighlight@prolog%
    \fi
  \fi
  % Some housekeeping...
  \global\predicate@prolog@false%
}

% helper macros
\newcommand\detectTypeAndHighlight@prolog
{%
  % First, assume that we have an atom.
  \def\lst@thestyle{\PrologAtomStyle}%
  % Test whether we have a predicate and modify the style accordingly.
  \ifpredicate@prolog@%
    \def\lst@thestyle{\PrologPredicateStyle}%
  \else
    % Test whether we have a predicate and modify the style accordingly.
    \expandafter\splitfirstchar@prolog\expandafter{\the\lst@token}%
    % Check whether the identifier starts by an underscore.
    \expandafter\ifx\@testChar@prolog\underscore@prolog%
      % Check whether the identifier is '_' (anonymous variable)
      \ifnum\lst@length=1%
        \let\lst@thestyle\PrologAnonymVarStyle%
      \else
        \let\lst@thestyle\PrologVarStyle%
      \fi
    \else
      % Check whether the identifier starts by a capital letter.
      \currentchar@prolog=65
      \loop
        \expandafter\ifnum\expandafter`\@testChar@prolog=\currentchar@prolog%
          \let\lst@thestyle\PrologVarStyle%
          \let\iterate\relax
        \fi
        \advance \currentchar@prolog by 1
        \unless\ifnum\currentchar@prolog>90
      \repeat
    \fi
  \fi
}
\newcommand\splitfirstchar@prolog{}
\def\splitfirstchar@prolog#1{\@splitfirstchar@prolog#1\relax}
\newcommand\@splitfirstchar@prolog{}
\def\@splitfirstchar@prolog#1#2\relax{\def\@testChar@prolog{#1}}

% helper macro for () delimiters
\def\beginlstdelim#1#2%
{%
  \def\endlstdelim{\PrologOtherStyle #2\egroup}%
  {\PrologOtherStyle #1}%
  \global\predicate@prolog@false%
  \withinparens@prolog@true%
  \bgroup\aftergroup\endlstdelim%
}

% language name
\newcommand\lang@prolog{Prolog-pretty}
% ``normalised'' language name
\expandafter\lst@NormedDef\expandafter\normlang@prolog%
  \expandafter{\lang@prolog}

% language definition
\expandafter\expandafter\expandafter\lstdefinelanguage\expandafter%
{\lang@prolog}
{%
  language            = Prolog,
  keywords            = {},      % reset all preset keywords
  showstringspaces    = false,
  alsoletter          = (,
  % alsodigit           = +,
  alsoother           = @$,
  % moredelim           = **[is][{(}{)}],
  moredelim           = **[is][\beginlstdelim{(}{)}]{(}{)},
  MoreSelectCharTable =
    \lst@DefSaveDef{`(}\opparen@prolog{\global\predicate@prolog@true\opparen@prolog},
}

% Hooking into listings to test each ``identifier''
\newcommand\@ddedToOutput@prolog\relax
\lst@AddToHook{Output}{\@ddedToOutput@prolog}

\lst@AddToHook{PreInit}
{%
  \ifx\lst@language\normlang@prolog%
    \let\@ddedToOutput@prolog\@testChar@prolog%
  \fi
}

\lst@AddToHook{DeInit}{\renewcommand\@ddedToOutput@prolog{}}

\makeatother
%
% --- end of ugly internals ---


% --- definition of a custom style similar to that of Pygments ---
% custom colors
\definecolor{PrologPredicate}{RGB}{000,031,255}
\definecolor{PrologVar}      {RGB}{000,031,255}
\definecolor{PrologAnonymVar}{RGB}{000,127,000}
\definecolor{PrologAtom}     {RGB}{182,000,000}
\definecolor{PrologComment}  {RGB}{063,128,127}
\definecolor{PrologOther}    {RGB}{000,000,000}

% redefinition of user macros for Prolog style
\renewcommand\PrologPredicateStyle{\color{PrologPredicate}}
\renewcommand\PrologVarStyle{\color{PrologVar}}
\renewcommand\PrologAnonymVarStyle{\color{PrologAnonymVar}}
\renewcommand\PrologAtomStyle{\color{PrologAtom}}
\renewcommand\PrologCommentStyle{\itshape\color{PrologComment}}
\renewcommand\PrologOtherStyle{\color{PrologOther}}

% custom style definition
\lstdefinestyle{Prolog-pygsty}
{
  language     = Prolog-pretty,
  upquote      = true,
  stringstyle  = \PrologAtomStyle,
  commentstyle = \PrologCommentStyle,
  literate     =
    {:-}{{\PrologOtherStyle $\leftarrow$\,}}2
    {,}{{\PrologOtherStyle ,}}2
    {.}{{\PrologOtherStyle .}}1
    {/}{{\PrologOtherStyle $\conc$}}2
%    {;}{{\PrologOtherStyle ,}}1
    {-}{{\PrologOtherStyle \$}}1
    {!}{{\PrologOtherStyle $\emp$}}1
    {+}{{\PrologOtherStyle $\lnot$}}1
    {^}{{\PrologOtherStyle $\neq$}}1
    {;}{{\PrologOtherStyle ;}}1
}

% global settings
\lstset
{
  captionpos = below,
  frame      = single,
  columns    = fullflexible,
  basicstyle = \ttfamily,
  escapeinside={(;}{;)},
}
%
% % write some sample code to an external file
% \begin{filecontents*}{sample.pl}
% somePredicate(_, B) :-
%     arbitraryPredicate(A, _variable, 1, 2),
%     predicateWithAtom(someAtom),
%     anotherPredicate(B, someAtom, myPredicate(A, _)),
%     findall(X, ('testString'(X), myPredicate(A, X)), L1),
%     member(A, L1),
%     !.
%     /*
%     block comment: blah blah blah
%     */
%     % to-end-of-line comment: blah blah blah
% \end{filecontents*}



  % \begin{lstlisting}[frame=none,mathescape,style=Prolog-pygsty,label=lst:allA]
  %   Q :- R(e_1), $\ldots$, R(e_i), ^ R(e_i+1), $\ldots$, ^ R(e_n)
  % \end{lstlisting}
  %
%   \begin{lstlisting}[basicstyle=\ttfamily, mathescape]
% $\delta$(Z, $\varepsilon$, $\mbox{\textdollar}$S) = (R, $\varepsilon$)
% $\delta$(Z, $\varepsilon$, $\$$S) = (R, $\varepsilon$)
% \end{lstlisting}

